Common Randomness Generation from Sources with Infinite Polish Alphabet

We investigate the problem of common randomness (CR) generation in the basic two-party communication setting in which a sender and a receiver aim to agree on a common random variable with high probability. The terminals observe independent and identically distributed (i.i.d.) samples of sources with an arbitrary distribution defined on a Polish alphabet and are allowed to communicate as little as possible over a noisy, memoryless channel. We establish single-letter upper and lower bounds on the CR capacity for the specified model. The derived bounds hold with equality except for at most countably many points where discontinuity issues might arise.

==> figures/Gaussian_MIMO.tex <==
\tikzstyle{farbverlauf} = [ top color=white, bottom color=white!80!gray]
\tikzstyle{vectorarrow} = [thick, decoration={markings,mark=at position
   1 with {\arrow[semithick]{open triangle 60}}},
   double distance=1.4pt, shorten >= 5.5pt,
   preaction = {decorate},
   postaction = {draw,line width=1.4pt, white,shorten >= 4.5pt}]
\tikzstyle{block} = [draw,top color=white, bottom color=white!80!gray, rectangle, rounded corners,
minimum height=2em, minimum width=2.5em]
\tikzstyle{input} = [coordinate]
\tikzstyle{sum} = [draw, circle,inner sep=0pt, minimum size=2mm,  thick]
\tikzstyle{arrow}=[draw,->] %{Latex[length=3mm]},
\scalebox{.87}{
\begin{tikzpicture}[auto, node distance=2cm,>=latex']
\node[] (M) {$M$};
\node[block,right=.4cm of M] (enc) {Encoder};
\node[block,right=.7cm of enc] (channel) {\large$\mathbf{H}$};
\node[sum, right=.7cm of channel] (sum) {$+$};
\node[block, right=.7cm of sum] (dec) {Decoder};
\node[right=.4cm of dec] (Mhat) {\begin{tabular}{c} Is $M^\prime$ sent? \\ Yes or No? \end{tabular}};
\node[above=.5cm of sum] (noise) {$\boldsymbol{\xi}$};
\draw[->] (M)--(enc);
\draw[vectorarrow] (enc) --node[above]{$\boldsymbol{x}$} (channel);
\draw[vectorarrow] (channel) -- (sum);
\draw[vectorarrow] (noise) -- (sum);
\draw[vectorarrow] (sum) -- node[above]{$\boldsymbol{y}$} (dec);
\draw[->] (dec) -- (Mhat) {};
\end{tikzpicture}}
